GraVoS: Voxel Selection for 3D Point-Cloud Detection

3D object detection within large 3D scenes is challenging not only due to the sparsity and irregularity of 3D point clouds, but also due to both the extreme foreground-background scene imbalance and class imbalance. A common approach is to add ground-truth objects from other scenes. Differently, we propose to modify the scenes by removing elements (voxels), rather than adding ones. Our approach selects the "meaningful" voxels, in a manner that addresses both types of dataset imbalance. The approach is general and can be applied to any voxel-based detector, yet the meaningfulness of a voxel is network-dependent. Our voxel selection is shown to improve the performance of several prominent 3D detection methods.

==> tables/ablation_dropout.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{l |c c c| c c c| c c c|  c}
    \hline
        Class & \multicolumn{3}{c}{Car}  & \multicolumn{3}{|c}{Cyclist} & \multicolumn{3}{|c|}{Pedestrian} & Avg.  \\ \hline
        Category & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &   \\ \hline
        Drop 60\% & 88.24 & 80.05 & 77.37 & 71.64 & 58.80 & 55.66 & 53.22 & 49.25 & 46.09 & 64.48 \\ \hline
        Drop 50\% & 89.68 & 80.88 & 78.27 & 77.70 & 62.48 & 59.06 & 55.38 & \textbf{50.76} & \textbf{47.33} & 66.84 \\ \hline
        Drop 40\% & \textbf{89.94} & 81.25 & 78.47 & 76.91 & 63.34 & 59.64 & 54.62 & 49.67 & 46.10 & 66.66 \\ \hline
        Drop 30\% & 89.87 & 81.22 & 78.41 & \textbf{80.39} & 64.38 & 60.61 & 53.36 & 48.84 & 44.79 & 66.87 \\ \hline
        Drop 20\% & 88.57 & \textbf{81.59} & \textbf{78.69} & 80.30 & 63.39 & 59.60 & \textbf{55.47} & 50.29 & 46.41 & 67.15 \\ \hline
        Drop 10\% & 89.91 & 81.41 & 78.51 & 80.24 & \textbf{64.47} & \textbf{60.83} & 55.23 & 50.00 & 45.61 & \textbf{67.36} \\ \hline
    \end{tabular}
\vspace{1pt}
\caption{Dropout ablation study using SECOND model on 3D detection benchmark.}
\label{tab:ablation_dropout}
\end{table*}

==> tables/ablation_thresholds.tex <==
\begin{table*}[!ht]
    \centering
    \small
    \begin{tabular}{l |c c c| c c c| c c c|  c}
    \hline
        Class & \multicolumn{3}{c}{Car}  & \multicolumn{3}{|c}{Cyclist} & \multicolumn{3}{|c|}{Pedestrian} & Avg.  \\ \hline
        Category & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &   \\ \hline
        SECOND \cite{second} & \textbf{90.79} & \textbf{81.87} & \textbf{78.75} & 81.85 & 65.42 & 61.26 & 54.90 & 49.84 & 45.15 & 67.76  \\ \hline
        l: \textbf{M}, ~~ e: \textbf{M} & 90.00 & 81.52 & 78.51 & 84.21 & 66.10 & 61.91 & 55.33 & 50.50 & 46.18 & 68.25 \\ \hline
        l: \textbf{M}, ~~ e: \textbf{MD} & 90.23 & 81.41 & 78.31 & 81.35 & 65.19 & 61.17 & 56.37 & 50.60 & 45.60 & 67.80 \\ \hline
        l: \textbf{M}, ~~ e: \textbf{T-$50$} & 90.24 & 81.27 & 78.10 & 81.87 & 64.13 & 60.20 & 55.11 & 49.73 & 45.29 & 67.33 \\ \hline
        l: \textbf{MD}, \,e: \textbf{M} & 90.08 & 81.39 & 78.44 & 81.07 & 63.99 & 60.10 & 57.69 & 51.93 & 47.39 & 68.01 \\ \hline
        l: \textbf{MD}, \,e: \textbf{MD} & 90.75 & 81.74 & 78.57 & 83.41 & \textbf{66.54} & 62.45 & 55.69 & 50.20 & 45.99 & 68.37 \\ \hline
        l: \textbf{MD}, \,e: \textbf{T-$50$} & 90.39 & 81.68 & 78.55 & 82.97 & 66.06 & 62.16 & 55.58 & 49.85 & 45.41 & 68.07 \\ \hline
        l: \textbf{T-$50$}, e: \textbf{M} & 89.53 & 81.06 & 78.07 & \textbf{84.36} & 66.41 & \textbf{62.61} & 57.75 & 51.99 & 47.54 & \textbf{68.81} \\ \hline
        l: \textbf{T-$50$}, e: \textbf{MD} & 90.54 & 81.38 & 78.41 & 83.13 & 65.86 & 61.63 & 56.38 & 50.80 & 46.10 & 68.25 \\ \hline
        l: \textbf{T-$50$}, e: \textbf{T-$30$} & 90.44 & 81.50 & 78.46 & 81.38 & 63.59 & 59.66 & \textbf{58.78} & \textbf{52.62} & \textbf{48.08} & 68.28 \\ \hline
        l: \textbf{T-$30$}, e: \textbf{T-$50$} & 90.63 & 81.78 & 78.60 & 83.75 & 65.29 & 61.33 & 55.48 & 49.61 & 45.42 & 67.99 \\ \hline
    \end{tabular}
\vspace{1pt}
\caption{Voxel selection threshold methods for late and early detector ablation studies. We abbreviate the late and early detector as l and e, respectively. For the selection methods: \textbf{M} refers to mean, \textbf{MD} to median, and \textbf{T-$n$} refers to top-k where $n/80$ represents the inter-detector-ratio value. The results for SECOND \cite{second} is provided as baseline.}
\label{tab:ablation_thresholds}
\end{table*}

==> tables/ablation_topk.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l |c c c| c c c| c c c|  c}
    \hline
        Class & \multicolumn{3}{c}{Car}  & \multicolumn{3}{|c}{Cyclist} & \multicolumn{3}{|c|}{Pedestrian} & Avg.  \\ \hline
        Category & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &   \\ \hline
        $\nu_{idr}$ 30/80 & 89.89 & 81.42 & 78.44 & 81.31 & 64.05 & 60.36 & 56.16 & 50.21 & 46.36 & 67.58 \\ \hline
        $\nu_{idr}$ 40/80 & 90.30 & 81.50 & 78.51 & 84.41 & 65.48 & 61.38 & 56.27 & 50.45 & 46.14 & 68.27 \\ \hline
        $\nu_{idr}$ 50/80 & 89.97 & 81.26 & 78.32 & \textbf{85.29} & \textbf{66.78} & \textbf{63.16} & 55.81 & 50.22 & 45.96 & \textbf{68.53} \\ \hline
        $\nu_{idr}$ 55/80 & 90.28 & 81.51 & 78.49 & 82.45 & 65.46 & 60.76 & 55.76 & 50.70 & 46.17 & 67.95 \\ \hline
        $\nu_{idr}$ 60/80 & 90.41 & 81.45 & 78.30 & 81.17 & 63.69 & 59.58 & \textbf{57.06} & \textbf{50.99} & \textbf{46.89} & 67.73 \\ \hline
        $\nu_{idr}$ 65/80 & 89.70 & 81.07 & 78.08 & 83.06 & 64.58 & 60.48 & 55.93 & 50.33 & 46.33 & 67.73  \\ \hline
        $\nu_{idr}$ 70/80 & \textbf{90.95} & 81.72 & 78.57 & 83.91 & 65.43 & 61.42 & 56.40 & 50.78 & 46.54 & 68.41 \\ \hline
        $\nu_{idr}$ 75/80 & 89.88 & 81.52 & 78.44 & 83.50 & 65.47 & 61.69 & 56.79 & 50.74 & 46.29 & 68.26 \\ \hline
        $\nu_{idr}$ 80/80 & 90.67 & \textbf{81.78} & \textbf{78.67} & 83.72 & 66.17 & 62.36 & 56.24 & 50.73 & 45.95 & 68.48 \\ \hline
    \end{tabular}
\vspace{1pt}
\caption{Inter-detector-ratio ($\nu_{idr}$), with a fixed Voxel selection ratio ($\nu_{vs}$) of 0.8, ablation study for SECOND model on 3D detection benchmark.}
\label{tab:ablation_topk}
\end{table*}

==> tables/ablation_vs.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l |c c c| c c c| c c c|  c}
    \hline
        Class & \multicolumn{3}{c}{Car}  & \multicolumn{3}{|c}{Cyclist} & \multicolumn{3}{|c|}{Pedestrian} & Avg.  \\ \hline
        Category & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &   \\ \hline
        $\nu_{vs}$ 0.4 & 90.02 & 81.23 & 78.24 & 75.50 & 59.88 & 56.38 & 50.42 & 45.15 & 40.71 & 64.17 \\ \hline
        $\nu_{vs}$ 0.5 & \textbf{90.72} & \textbf{81.98} & \textbf{78.70} & 81.30 & 64.06 & 60.04 & 51.45 & 46.06 & 41.82 & 66.24 \\ \hline
        $\nu_{vs}$ 0.6 & 90.63 & 81.92 & 78.68 & 80.58 & 64.69 & 60.40 & 53.70 & 48.92 & 44.79 & 67.15 \\ \hline
        $\nu_{vs}$ 0.7 & 89.74 & 81.38 & 78.41 & 79.91 & 63.68 & 60.39 & 56.38 & 51.16 & \textbf{47.18} & 67.58 \\ \hline
        $\nu_{vs}$ 0.8 & 89.97 & 81.26 & 78.32 & \textbf{85.29} & \textbf{66.78} & \textbf{63.16} & 55.81 & 50.22 & 45.96 & \textbf{68.53} \\ \hline
        $\nu_{vs}$ 0.9 & 90.03 & 81.54 & 78.39 & 82.46 & 65.56 & 61.95 & \textbf{57.53} & \textbf{51.79} & 47.17 & 68.49 \\ \hline
    \end{tabular}
\vspace{1pt}
\caption{Voxel selection ratio ($\nu_{vs}$) ablation study, with a fixed inter-detector-ratio ($\nu_{idr}$) of 50/80 on 3D detection benchmark, using SECOND model.}
\label{tab:ablation_vs}
\end{table*}

==> tables/mechanisms_ablation.tex <==
\begin{table*}[!ht]
    \centering
    \small
    \begin{tabular}{l |c c c| c c c| c c c|  c}
    \hline
        Class & \multicolumn{3}{c}{Car}  & \multicolumn{3}{|c}{Cyclist} & \multicolumn{3}{|c|}{Pedestrian} & Avg.  \\ \hline
        Category & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &   \\ \hline
        SECOND \cite{second} & \textbf{90.79} & \textbf{81.87} & \textbf{78.75} & 81.85 & 65.42 & 61.26 & 54.90 & 49.84 & 45.15 & 67.76  \\ \hline
        l: \textbf{M}, ~~ e: \textbf{M} & 90.00 & 81.52 & 78.51 & 84.21 & 66.10 & 61.91 & 55.33 & 50.50 & 46.18 & 68.25 \\ \hline
        l: \textbf{M}, ~~ e: \textbf{MD} & 90.23 & 81.41 & 78.31 & 81.35 & 65.19 & 61.17 & 56.37 & 50.60 & 45.60 & 67.80 \\ \hline
        l: \textbf{M}, ~~ e: \textbf{T-$50$} & 90.24 & 81.27 & 78.10 & 81.87 & 64.13 & 60.20 & 55.11 & 49.73 & 45.29 & 67.33 \\ \hline
        l: \textbf{MD}, \,e: \textbf{M} & 90.08 & 81.39 & 78.44 & 81.07 & 63.99 & 60.10 & 57.69 & 51.93 & 47.39 & 68.01 \\ \hline
        l: \textbf{MD}, \,e: \textbf{MD} & 90.75 & 81.74 & 78.57 & 83.41 & \textbf{66.54} & 62.45 & 55.69 & 50.20 & 45.99 & 68.37 \\ \hline
        l: \textbf{MD}, \,e: \textbf{T-$50$} & 90.39 & 81.68 & 78.55 & 82.97 & 66.06 & 62.16 & 55.58 & 49.85 & 45.41 & 68.07 \\ \hline
        l: \textbf{T-$50$}, e: \textbf{M} & 89.53 & 81.06 & 78.07 & \textbf{84.36} & 66.41 & \textbf{62.61} & 57.75 & 51.99 & 47.54 & \textbf{68.81} \\ \hline
        l: \textbf{T-$50$}, e: \textbf{MD} & 90.54 & 81.38 & 78.41 & 83.13 & 65.86 & 61.63 & 56.38 & 50.80 & 46.10 & 68.25 \\ \hline
        l: \textbf{T-$50$}, e: \textbf{T-$30$} & 90.44 & 81.50 & 78.46 & 81.38 & 63.59 & 59.66 & \textbf{58.78} & \textbf{52.62} & \textbf{48.08} & 68.28 \\ \hline
        l: \textbf{T-$30$}, e: \textbf{T-$50$} & 90.63 & 81.78 & 78.60 & 83.75 & 65.29 & 61.33 & 55.48 & 49.61 & 45.42 & 67.99 \\ \hline
    \end{tabular}
\vspace{1pt}
\caption{\textbf{Different mechanisms choices for the early and late detectors.} We abbreviate the late and early detector as l and e, respectively. 
For the selection methods: \textbf{M} refers to mean, 
\textbf{MD} to median, 
and \textbf{T-$n$} refers to top-k where $n/80$ represents the intra-detector-ratio value. 
The results for SECOND~\cite{second} is provided as baseline.}
\label{tab:mechanisms_ablation}
\end{table*}

==> tables/sota_comparison_backup.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l |c c c| c c c| c c c|  c}
    \hline
        Class & \multicolumn{3}{c}{Car}  & \multicolumn{3}{|c}{Cyclist} & \multicolumn{3}{|c|}{Pedestrian} & Avg.  \\ \hline
        Category & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &   \\ \hline
        SECOND \cite{second} & \textbf{90.73} & \textbf{81.87} & \textbf{78.75} & 81.85 & 65.42 & 61.26 & 54.9 & 49.84 & 45.15 & 67.75  \\
        \cite{second} + ft & 90.05 & 81.50 & 78.55 & 81.52 & 65.47 & 61.65 & 54.74 & 49.44 & 44.57 & 67.50  \\ 
        \cite{second} + Ours & 89.53 & 81.06 & 78.07 & \textbf{84.36} & \textbf{66.41} & \textbf{62.61} & \textbf{57.75} & \textbf{51.99} & \textbf{47.54} & \textbf{68.81}  \\ 
        \hline
        Voxel R-CNN \cite{voxelrcnn} & 92.62 & 85.13 & 82.73 & 89.83 & 72.49 & 68.87 & 66.94 & 59.88 & 54.95 & 74.83  \\ 
        \cite{voxelrcnn} + ft & \textbf{92.69} & 85.25 & \textbf{82.85} & 90.55 & \textbf{ 73.06 }& \textbf{69.62} & 65.64 & 59.58 & 54.75 & 74.89   \\ 
        \cite{voxelrcnn} + Ours & 92.42 & \textbf{85.41} & 82.84 & \textbf{91.93} & 72.91 & 68.38 & \textbf{68.42} & \textbf{61.56} & \textbf{56.68} & \textbf{75.62}  \\ 
        \hline
        Part-$A^2$ \cite{parta2} & 91.91 & 82.67 & 80.23 & 89.44 & 71.79 & 67.79 & 65.41 & 58.42 & 53.60 & 73.47  \\ 
        \cite{parta2} + ft & \textbf{92.06} & \textbf{82.71} & \textbf{81.78} & 88.86 & 72.86 & 68.53 & \textbf{66.00} & 58.71 & 53.86 & 73.93  \\ 
        \cite{parta2} + Ours & 91.69 & 82.58 & 81.67 & \textbf{90.51} & \textbf{74.02} & \textbf{69.71} & 65.88 & \textbf{59.57} & \textbf{54.52} & \textbf{74.46}  \\ 
        \hline
        CenterPoint \cite{yin2021center} & \textbf{89.58} & \textbf{82.08} & \textbf{79.57} & 80.27 & 62.85 & 60.14 & 56.86 & 53.18 & 49.73 & 68.25  \\ 
        \cite{yin2021center} + ft &   &  &  &  &  &  &  &  &  &  \\ 
        \cite{yin2021center} + Ours & 88.74 & 81.73	& 79.52	& \textbf{83.4} & \textbf{64.81} & \textbf{61.41} & \textbf{58.01} & \textbf{54.65} & \textbf{50.95} & \textbf{69.25}  \\ 
        \hline
    \end{tabular}
\vspace{1pt}
\caption{Comparison of 3D detection AP performance on the KITTI dataset for SOTA methods. We compare our reproduction of the original method's performance, with a baseline of continuing to fine tune the detector without augmentations (+ft), and with gradient-based voxel selection augmentation (Ours). Results are reported for the Easy, Moderate (Mod.) and Hard categories on the Car, Cyclist, and Pedestrian classes.}
\label{tab:sota_comparison}
\end{table*}

==> tables/sota_comparison_sup_ft.tex <==
\begin{table*}[t]
    \centering
    \small
    % \setlength{\tabcolsep}{4pt}
    \begin{tabular}{|l |c c c| c c c| c c c| c c c c | c|}
    \hline
          & \multicolumn{3}{c}{\em Car}  & \multicolumn{3}{|c}{\em Cyclist} & \multicolumn{3}{|c|}{\em Pedestrian} & \multicolumn{4}{c|}{Average} \\
        Method & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Mod.} & \multicolumn{1}{c|}{Hard} &  
        \multicolumn{1}{c}{\em Car} & \multicolumn{1}{c}{\em Cyc.} & \multicolumn{1}{c}{\em Ped.}  & \multicolumn{1}{c|}{All} \\   \hline
    \hline
        SECOND \cite{second} & \textbf{90.79} & \textbf{81.87} & \textbf{78.75} & 81.85 & 65.42 & 61.26 & 54.90 & 49.84 & 45.15 & \textbf{83.80} & 69.51 & 49.96 & 67.76 \\
        SECOND\dag & 90.05 & 81.50 & 78.55 & 81.52 & 65.47 & 61.65 & 54.74 & 49.44 & 44.57 & 83.37 & 69.55 & 49.58 & 67.50  \\
        Ours & 89.53 & 81.06 & 78.07 & \textbf{84.36} & \textbf{66.41} & \textbf{62.61} & \textbf{57.75} & \textbf{51.99} & \textbf{47.54} & 82.89 & \textbf{71.13} & \textbf{52.43} & \textbf{68.81} \\
        \hline
        Voxel R-CNN \cite{voxelrcnn} & 92.62 & 85.13 & 82.73 & 89.83 & 72.49 & 68.87 & 66.94 & 59.88 & 54.95 & 86.83 & 77.06 & 60.59 & 74.83 \\ 
        Voxel R-CNN\dag & \textbf{92.69} & 85.25 & \textbf{82.85} & 90.55 & \textbf{ 73.06 }& \textbf{69.62} & 65.64 & 59.58 & 54.75 & \textbf{86.93} & 77.74 & 59.99 & 74.89   \\
        Ours & 92.40 & \textbf{85.41} & 82.84 & \textbf{91.97} & 72.98 & 68.37 & \textbf{68.52} & \textbf{61.63} & \textbf{56.71} & 86.88 & \textbf{77.77} & \textbf{62.29} & \textbf{75.65} \\ 
        \hline
        Part-$A^2$ \cite{parta2} & 91.88 & 82.64 & 80.21 & 89.45 & 71.71 & 67.74 & 65.37 & 58.43 & 53.62 & 84.91 & 76.30 & 59.14 & 73.45 \\
        Part-$A^2$\dag & \textbf{92.06} & \textbf{82.71} & \textbf{81.78} & 88.86 & 72.86 & 68.53 & \textbf{66.00} & 58.71 & 53.86 & \textbf{85.52} & 76.75 & 59.52 & 73.93  \\ 
        Ours & 91.68 & 82.58 & 81.67 & \textbf{90.64} & \textbf{74.03} & \textbf{69.64} & 65.82 & \textbf{59.58} & \textbf{54.55} & 85.31 & \textbf{78.10} & \textbf{59.98} & \textbf{74.47} \\
        \hline
    \end{tabular}
\vspace{1pt}
\caption{
{\bf Training scheme comparison on the 3D detection benchmark. } 
Each detector with $\dag$ represents the detector after continuing to train with the same number of epochs, learning rate, and scheduler as in our method but without our voxel selection module.
}
\label{tab:ft_comparison_sup}
\end{table*}
